Toward Real World Stereo Image Super-Resolution via Hybrid Degradation Model and Discriminator for Implied Stereo Image Information

Real-world stereo image super-resolution has a significant influence on enhancing the performance of computer vision systems. Although existing methods for single-image super-resolution can be applied to improve stereo images, these methods often introduce notable modifications to the inherent disparity, resulting in a loss in the consistency of disparity between the original and the enhanced stereo images. To overcome this limitation, this paper proposes a novel approach that integrates a implicit stereo information discriminator and a hybrid degradation model. This combination ensures effective enhancement while preserving disparity consistency. The proposed method bridges the gap between the complex degradations in real-world stereo domain and the simpler degradations in real-world single-image super-resolution domain. Our results demonstrate impressive performance on synthetic and real datasets, enhancing visual perception while maintaining disparity consistency. The complete code is available at the following \href{https://github.com/fzuzyb/SCGLANet}{link}.

==> chaps/acknowledgements.tex <==
\section*{Acknowledgements}
This work was supported by National Natural Science Foundation of China under Grant 62171133, in part by the Artificial Intelligence and Economy Integration Platform of Fujian Province, and the Fujian Health Commission under Grant 2022ZD01003. 

==> chaps/biographies.tex <==
\section*{Biographies}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/yuanbozhou.png}}]{Yuanbo Zhou} received his B.S. in Internet of Things from Fuzhou University in 2018. He is currently pursuing the Ph.D. degree with Fuzhou University. His main research interests are 3D vision, image super-resolution and model compressing.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/yuyangxue.jpg}}]{Yuyang Xue} received the B.S. degree in computer science from Fuzhou University, in 2016. He received the M.S. degree in computer science from University of Southampton, in 2018. He is currently pursuing the Ph.D. degree with University of Edinburgh. His research interests include machine learning and computer vision. He is an IEEE Graduate Student Member.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/xinlinzhang.jpg}}]{Xinlin Zhang} received her B.S. degree in 2016, and Ph.D. degree in 2022 from the Department of Electronic Science, Xiamen University, respectively. Her main research interests lie in signal processing, optimization, medical imaging, and artificial intelligence.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/zz.jpg}}]{Jiajun Zhang} received the B.S. degree in communication engineering from Fujian University of technology in 2021. He is pursuing the M.S. degree with Fuzhou University. His main research interests are image super-resolution and efficient image restoration.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/dengwei.png}}]{Wei Deng} received his M.S. degree in Computer software and theory from Fuzhou University in 2018. He is currently senior algorithm development engineer at Imperial Vision Technology. His main research interests are image restoration and generative adversarial network.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/nieruofeng.png}}]{Ruofeng Nie} received his B.S. in College of Biomedical Engineering and Instrument Science from Zhejiang University in 2019. He is currently an algorithm engineer in Fujian Imperial Vision Technology. His main research interests are image super-resolution, image enhancement, face generation and image segmentation.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/lanjunlin.png}}]{Junlin Lan} received his B.S. in Internet of Things from Fuzhou University in 2018. He is currently pursuing the Ph.D. degree with Fuzhou University. His main research interests is medical image processing.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/gaoqinquan.png}}]{Qinquan Gao} received the B.S. degree in automation and the M.S. degree in systems engineering from Xiamen University, China, in 2008 and 2010, respectively, and the Ph.D.degree from Imperial College London in 2014. He is currently an Associate Professor with Fuzhou University and founder of Imperial Vision Technology, working on image super-resolution, machine learning, biomedical image processing, and computer vision.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Biographies/tongtong.png}}]{Tong Tong} (Ph.D., 2015, Imperial College London; Research Fellow, 2016, MGH/Harvard Medical School) is a full professor in the College of Physics and Information Engineering at Fuzhou University. His research interests include machine learning, medical image analysis and computer aided diagnosis.
\end{IEEEbiography} 

==> figures/KITTIMB.tex <==
\begin{figure*}[!t]
\begin{center}
\scalebox{0.99}{
\begin{tabular}[b]{c@{ } c@{ } c@{ }  c@{ } c@{ } c@{ } c@{ } }


    \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2012/0_1_0.png} &
    \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2012/0_1_1.png} &
    \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2012/0_1_2.png} &
    \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2012/0_1_3.png} &
    \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2012/0_1_4.png} &
    \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2012/0_1_5.png} &
    \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2012/0_1_6.png}
   \\
   \vspace{0.1mm}
   \\



 \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2015/10_1_0.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2015/10_1_1.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2015/10_1_2.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2015/10_1_3.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2015/10_1_4.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2015/10_1_5.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/KITTI2015/10_1_6.png}
  \\

 \vspace{0.1mm}
 \\

 \includegraphics[width=.136\textwidth,valign=t]{figures/MB/3_1_0.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/MB/3_1_1.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/MB/3_1_2.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/MB/3_1_3.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/MB/3_1_4.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/MB/3_1_5.png} &
 \includegraphics[width=.136\textwidth,valign=t]{figures/MB/3_1_6.png} \\
 
\scriptsize~Bicubic    &
\scriptsize~RCAN~\cite{zhang2018image} &
\scriptsize~iPASSR~\cite{wang2021symmetric} & \scriptsize~SSRDE-FNet~\cite{dai2021feedback} &\scriptsize~NAFSSR-L ~\cite{chu2022nafssr} &\scriptsize~SCGLANet(ours)  & \scriptsize~GT\\



\end{tabular}}
\end{center}
\vspace{-1mm}
\caption{Visual results ($\times$4) achieved by different methods on the KITTI 2012~\cite{geiger2012we} (top), KITTI 2015~  \cite{geiger2015kitti} (center) and Middlebury \cite{scharstein2014high} (bottom) dataset.
}
\label{fig:kittimb}
\vspace{-3mm}
\end{figure*}


